FabricQA-Extractor: A Question Answering System to Extract Information from Documents using Natural Language Questions

Reading comprehension models answer questions posed in natural language when provided with a short passage of text. They present an opportunity to address a long-standing challenge in data management: the extraction of structured data from unstructured text. Consequently, several approaches are using these models to perform information extraction. However, these modern approaches leave an opportunity behind because they do not exploit the relational structure of the target extraction table. In this paper, we introduce a new model, Relation Coherence, that exploits knowledge of the relational structure to improve the extraction quality. We incorporate the Relation Coherence model as part of FabricQA-Extractor, an end-to-end system we built from scratch to conduct large scale extraction tasks over millions of documents. We demonstrate on two datasets with millions of passages that Relation Coherence boosts extraction performance and evaluate FabricQA-Extractor on large scale datasets.

==> sections/implementation.tex <==
\section{Implementation and Carpentry}
\label{sec:implementation}

Before the evaluation section, we present implementation details that greatly
impact the overall system performance.

\subsection{Carpentry}

%\mypar{Indexing documents} Documents are split into passages via the Chunker. We
%split documents by applying a sliding window over the text. The window size is
%100, leading to 100-word tokens. The slide is 50. We empirically demonstrate in
%the evaluation the positive effect of this decision.

\mypar{Question pre-processing} We choose Elasticsearch~\cite{elasticsearch} (ES) as the
information retrieval system. Before sending a question to ES, it is
pre-processed with Spacy~\cite{spacy2} to identify important tokens, such as
the Saxon genitive, which indicates possesion and has thus an important impact
on the meaning of questions. For example, default tokenizers will produce the
token 'John's'; with the pre-processing we seek to have 'John' and ''s' as
separate tokens. 

\mypar{Passage Re-ranking} Given two passages that contain the tokens in
the subject, we would like the passage matching exactly the subject phrase to
have a higher score. However, ES uses BM25 \cite{bm25, INR-019} to
score passages given a question and BM25 does not consider token order. We
therefore construct a compound bool query to ensure exact match (including
order) ranks higher. 

\mypar{Exposing model internal representations} Commoditization of machine
learning models means that many models are published as black boxes, which is
good for usability, but insufficient when access to their internal
representations is needed. We modify the RC model available on Hugging
Face~\cite{hugging_face} so we access its internal token vector representation,
which we use for training the reader.

\subsection{Hands-Free Setup}

\notera{explain how we choose parameters in this system and any design decision
aimed at minimizing the effort required to setting things up}




==> sections/old_fabricqa.tex <==
\section{\textsf{FabricQA}: Answer This}
\label{sec:fabricqa}

In this section, we present the architecture and components of
\textsf{FabricQA}, which together implement the \textsf{answer-this} primitive.
The architecture consists of an \emph{Chunker and Indexer}
(Section~\ref{subsec:chunkerindexer}) a \emph{Passage Ranker}
(Section~\ref{subsec:passageranker}) and an \emph{Answer Ranker}
(Section~\ref{subsec:answerranker}).

\subsection{Chunker and Indexer}
\label{subsec:chunkerindexer}

During the offline stage, the document corpora is indexed into a state of the
art information retrieval system. Documents are heterogeneous on their topics,
but also on their lenghts, paragraph structure, and formatting. We found that
indexing entire documents harmed the performance of the system. Instead, we
split each input document into passages of roughly the same size. A passage is
defined by the number of words it contains. This serves two purposes. First, the
answer to many questions is contained in individual sentences, so a passage is
sufficiently large to capture it. Second, passages conform to the input
restrictions of RC models, which \textsf{FabricQA} uses downstream, and that
cannot process larger documents without a loss in performance. For example,
BERT-based QA readers such as \cite{albert} do not accept passages longer than
512 tokens, and a single word is usually represented with more than one token,
according to the wordpiece algorithm~\cite{wordpiece}. We split passages into
200 words approximately and show evidence for this decision in the evaluation
section.

The chunker component of \textsf{FabricQA} merges paragraphs of documents and
read the documents as a stream of tokens. To chunk the stream, it uses a sliding
window, that ensures there is some overlap of tokens across neighboring
paragraphs.  Although this redundancy increases the storage footprint in the
information retrieval system, it also boosts the performance of the end to end
system because it ensures there is no context loss despite losing paragraph
boundaries.

Finally, during the offline stage, the Indexer component assigns an ID to each
passage and stores it along with the document it belongs to in the information
retrieval system.

\mypar{Note on information retrieval system} We assume the information retrieval
system can return the $K$ most relevant passages to an input query, along with
the ranking score associated to each passage. Most information retrieval systems
implement this functionality. 

\subsection{Passage Ranker}
\label{subsec:passageranker}

The \textsf{Passage Ranker} retrieves $K1$ passages from the information
retrieval system and forwards $K2$ passages downstream to the \textsf{Answer
Ranker}, where $K2 < K1$.  $K1$ is usually in the hundreds, while $K2$ in the
tens. The information retrieval system can return those passages fast because it
only uses \emph{syntactic} information to rank and retrieve passages. The
\textsf{Passage Ranker} uses \emph{semantic} information, as available through
language models, to narrow down the passages that get sent downstream to the
more computationally expensive \textsf{Answer Ranker}.

We designed the \textsf{Passage Ranker} in many different ways, and observed
many different proposals appearing in the related work over the last two years.
After extensive experimentation, we concluded that state of the art RC models
effectively subsume the role of a \textsf{Passage Ranker}. That is, the scores
they associate to the answers they provide already rank the passages according
to how likely they are to contain the right answer to the question. We exploit
this insight to implement the \textsf{Passage Ranker} as explained next.

\mypar{RC Model} An RC model takes as input a question and a passage and finds a
span of text in the passage that corresponds to the answer. It then returns the
text span and a score, $S_{best}$ associated to the confidence the model has in
that answer. Furthermore, state-of-the-art RC models return 'null' when they do
not find a valid text span in a passage. 

\mypar{Building a Passage Ranker off RC Model scores} We apply the RC model to
each passage obtained from the information retrieval system. Then, we normalize
the scores associated with each passage-answer using a simple \emph{margin
score}, defined as: $S_{margin} = S_{best} - S_{null}$. Then, this component
sends downstream the top-$K2$ passage-answer-question triples, those with the
highest $S_{margin}$. 

\subsection{Answer Ranker}
\label{subsec:answerranker}

The \textsf{Answer Ranker} is a neural network model that takes a question, $Q$,
passage $P$ and the answer provided by the Reader $A$ and returns a score that
indicates how likely $A$ is an answer to $Q$ given $P$. Each of the $K2$
passages from the \textsf{Passage Ranker} are fed to the \textsf{Answer Ranker}
and the top-$K3$ chosen\footnote{Note one can configure $K3=1$ to obtain the
best answer according to \textsf{FabricQA}. In general,
\textsf{FabricQA-Extractor} will obtain $K3>1$ and provide those candidate
answers to the Relation Coherence model.}.

$P$, $Q$, and $A$ are featurized into fixed-length vectors using BERT as the
language model. The resulting feature vectors are concatenated as shown in
\F\ref{fig:answer_ranker}.  $Q$ and $P$ are prefixed by a special token $<CLS>$
and there is a special end token, $<SEP>$, after which the answer is included.
The answer, $A$ is represented as a continuous span of tokens from $P_s$ to
$P_e$, which are the start and end token indicating the span of text in the
passage that corresponds to the answer.

\begin{figure}[h]
  \centering
  \includegraphics[width=\columnwidth]{img/answer_ranker}
  \caption{Schematic of the Answer ranker model}
  \label{fig:answer_ranker}
\end{figure}

The model uses the following vector representations:

\begin{myitemize}

\item{$\textbf{h}_{best}$}, vector representation for the answer. We concatenate
the answer start and end token vector along column to get the best answer
vector, i.e. $\textbf{h}_{best} = [BERT(P_s);BERT(P_e)]$. Where
$\text{BERT}(P_i)$ denotes the vector of token $P_i$ encoded by Bert.
%\[
%\textbf{h}_{best} = [BERT(P_s);BERT(P_e)]
%\]

\item{$\textbf{h}_{null}$}, is the vector representation for cases where no
answer is found, in which BERT returns the position of the start token, $<CLS>$. 
%vector representation for no answer. In case of no
%answer found, Bert reader returns the position of the start token $<CLS>$. So
%
%\[
%\textbf{h}_{null} = \text{BERT}(P_1)
%\]

\item{$\textbf{h}_{q}$}, is the vector representation of the question, computed
as the average of the vector representation of each token in $Q$:
$\textbf{h}_{q} = \frac{1}{m}\sum_{i=1}^{m}\text{BERT}(Q_i)$

%\[
%\textbf{h}_{q} = \frac{1}{m}\sum_{i=1}^{m}\text{BERT}(Q_i)
%\] 
\end{myitemize}

The model then obtains \textbf{h} by concatenating the previous vectors, $h =
[\textbf{h}_{best} ; \textbf{h}_{null} ; \textbf{h}_{q}]$, and then feeds it
into a
multilayer perceptron to compute the score: $S(Q,P,A) =
\textbf{w}_2^T(dropout(relu(\textbf{w}_1^T \textbf{h} + \textbf{b}_1))) +
\textbf{b}_2$, where $\textbf{w}_1, \textbf{w}_2, \textbf{b}_1, \textbf{b}_2$
are network parameters, $relu$ is the activation function, $dropout$ is used to
prevent overfitting and ";" is the column concatenation operator. 


%from the previous
%vectors and feeds it into a multilayer perceptron to compute a score for each
%$(Q, P, A)$ tuple.

%We then concatenate them along column to get one vector, \textbf{h} which is
%then fed to a neural network, or multilayer perceptron (MLP) to compute a score
%for each $(Q, P, A)$ tuple. 

%\begin{alignat*}{2}
%&S(Q, P, A) &&= MLP([\textbf{h}_{best} ; \textbf{h}_{null} ; \textbf{h}_{q}]) \\
%&			 &&= MLP(\textbf{h}) \\
%&	         &&= \textbf{w}_2^T(dropout(relu(\textbf{w}_1^T \textbf{h} + \textbf{b}_1))) + \textbf{b}_2
%\end{alignat*}

The \textsf{Answer Ranker} models the distance between the answer to the question and to
the null answer in an embedded space, $S(Q, P, A)$. Scores are assigned based on
the distance to question and null answer. We refer to \textbf{h} as answer
distance vector.

% and we are more confident with
%a $(Q, P, A)$ if its answer margin is higher. 

\mypar{Offline training} To train
Answer Ranker, for each Q, we need $N^+$ positive passages $P^+$ and $N^-$
negative passages $P^-$. We use cross-entropy loss, i.e. minimize

\begin{alignat*}{2}
&-\log Pr(Q, P^+, A^+ | Q) = -\frac{1}{N^+}\sum_{i=1}^{N^+}Pr(Q, P_{i}^+, A_{i}^+ | Q) \\
&=-\frac{1}{N^+}\sum_{i=1}^{N^+} \frac{\exp\left\{S(Q, P_i^+, A_i^+)\right\}}{\exp\left\{S(Q, P_i^+, A_i^+)\right\} + \sum_{j=1}^{N^-}\exp\left\{S(Q, P_j^-, A_j^-)\right\}}
\end{alignat*}

Where $Pr(Q, P^+, A^+ | Q)$ is the conditional probability of $(Q, P^+, A^+) $
given $Q$. We explain how to use distant supervision to collect a training
dataset for this model in Section~\ref{sec:implementation}.



==> sections/old_rq1.tex <==
\subsection{RQ1: IE as Question Answering}

\notefb{R1-D3 - In section 7.2, the description of the pipeline for the IE system built with DeepDive and details about running it are interesting, but I question whether comparing this system quantitatively is fair since it seems like its efficacy largely depends on the quality on the human-specified rules for identifying positive/negative sentences. How are the authors validating their set of rules? Another issue is that the section presents results only for a small sample from one dataset. The authors mention this is due to the large effort needed to run the pipeline for a relation. But results with other datasets and 1-2 more approaches, particularly a QA-based approach, are needed to demonstrate the efficacy of the proposed approach.}

\noteqi{
a)... but I question whether comparing this system quantitatively is fair... \\
> It is true that DeepDive will achieves better performance if more effort is spent on tuning the rules, but it relies much on domain experts to do that.\\
b)... How are the authors validating their set of rules? ...\\
> We use development dataset (same relationship but different subject/object pairs from test) to validate the set of rules. \\
c)... But results with other datasets and 1-2 more approaches ... \\
> Currently we compare IE and QA approach only on QA-ZRE, we can try BioNLP as well.
}

In this section we evaluate the central hypothesis of this  paper which is that
question answering has advantages with respect to state of the art information
extraction pipelines.

To do that, we build an information extraction pipeline, \textsf{IE-system}, and
compare its performance with \textsf{FabricQA-Extractor} using a sample of
relationships from \textsf{QA-ZRE-Open} (see Table~\ref{table:sample-zre}).

\input{tables/sample-qa-zre}

\subsubsection{Building \textsf{IE-System}}

We build an information extraction pipel\-ine using DeepDive~\cite{deepdive}, a
state of the art framework for doing information extraction from text.  Deepdive
\cite{deepdive} is a representative IE framework that extracts relations from
text, and does statistical inference and learning at scale to improve the
results quality by using relational databases. Deepdive-based applications
achieved best results in the TAC-KBP 2014 and 2017 competition
\cite{stanford-2014-sf, stanford-tac-2017}. 

\textsf{IE-System} implements a pipeline with the following stages. For each
relationship,

\begin{myitemize}

\item{Collect candidate tuples}. Each relationship indicates a pair of entity
type, and we extract all entity pairs in each sentence of the corpus matching
the entity type pair. We also extract the corresponding sentences.

\item{Entity link}. We link the tuples in QA-ZRE-Open to candidate tuples so
that we can get the corresponding sentences as features.

\item{Collect training data}. We write rules to identify positive and negative
sentences for each tuple in QA-ZRE-Open train set. Positive sentences contain
the relationship in the tuple; those that do not contain it are labeled as
Negative.

\item{Train and infer}. We generate features for each sentence using Deepdive
API and then train a model using Deepdive commands which infer in the test data
as well.

\end{myitemize}

Note that the entire pipeline above is specific to each relationship. If we ask
a question about a new relationship, then the pipeline needs to be rebuilt for
that relationship to obtain good results. Because this is so time-consuming, we
only use 5 relationships from \textsf{QZ-ZRE-Open} in this experiment (see
Table~\ref{table:sample-zre}).
 
\subsubsection{Details on \textsf{IE-System} setup}

\mypar{Collect candidate tuples} Deepdive relies on named entity recognition
(NER) package to extract candidates, and uses Stanford CoreNLP \cite{core-nlp}
as default. We use Spacy\cite{spacy2} instead because it offers more NER tags
and is considered the state of the art library. With Spacy we could recognize
entities in 3 out of the 5 relationships in the benchmark (\emph{industry} and
\emph{profession} were not recognized by either CoreNLP or Spacy). 

\mypar{Entity link} To link entity mentions in candidate tuples to entities in
QA-ZRE-Open train set, we use both fuzzy match so that pairs with an F1 socre
above $0.5$ match. Because we do not know which entity is subject or object
in a candidate, we further swap the entities in a candidate to link them.

%\notera{the following is unclear}
For dev/test data, we link subject to one the entities in the candidate tuples, 
and retrieve top 10 candidates.

\mypar{Collect training data} If a candidate tuple exactly matches a tuple in the
QA-ZRE-Open train set, we label the sentence
corresponding to the candidate tuple as positive. If it fuzzy matches the tuple,
then we use additional rules to boost confidence, \eg for the employer relationship,
if the sentence contains words like "work", "worked", "join", we label it as
positive. We sample 3 positive candidates for each train tuple, always prefering
exact matches if available. To collect negative examples, we choose candidates
in which only one entity matches. We sample 6 negative passages.

\subsubsection{Results}

The results for both \textsf{IE-System} and \textsf{FabricQA-Extractor} are
shown in Table~\ref{table:deepdive}. We comment on two aspects, quantitative
results, and more importantly, the qualitative effort invested in making each
system work.

\begin{table}[ht]
\scalebox{0.9}{
\begin{tabular}{|l|l|l|l|l|l|l|}
\hline
\multirow{2}{*}{\textbf{Relationship}} & \multicolumn{2}{l|}{\textsf{IE-System}} & \multicolumn{2}{l|}{\textsf{\begin{tabular}[c]{@{}l@{}}FabricQA\\ Extractor\end{tabular}}} & \multicolumn{2}{l|}{\textbf{Difference}} \\ \cline{2-7} 
                                       & \textbf{EM}        & \textbf{F1}       & \textbf{EM}                                  & \textbf{F1}                                 & \textbf{EM}         & \textbf{F1}        \\ \hline
employer                               & 6.8                & 11.0              & 11.8                                         & 37.3                                        & 5.0                 & 26.4               \\ \hline
illustrator                            & 3.0                & 4.0               & 80.6                                         & 83.8                                        & 77.6                & 79.8               \\ \hline
production company                     & 3.1                & 4.3               & 59.7                                         & 71.9                                        & 56.6                & 67.6               \\ \hline
\end{tabular}
}
\caption{Performance of \textsf{IE-System} and \textsf{FabricQA-Extractor}} 
\label{table:deepdive}
\end{table}

\mypar{Quantitative Results} Table \ref{table:deepdive} shows that despite being
trained for each relationship specifically, the performance of
\textsf{IE-System} is lower than \textsf{FabricQA-Extractor}, which was not
specifically trained for these relationships. The performance gap is a testament
to the progress the natural language community has made over the last 5 years in
advancing he state of the art in language modeling, with embedding models such
as BERT~\cite{bert} that enabled advanced RC models such as the ones used as
part of \textsf{FabricQA-Extractor}. Still, leveraging all that progress to
address the information extraction problem is not straightforward, as we show in
this paper.

\notefb{R1-D4 - For the qualitative results in Section 7.2.3, please specify how long it takes to run the pipeline (e.g., 3 hours). If the time breakdown per stage is interesting, you could include that information too.}

\noteqi{It is ok to include the time}

\mypar{Qualitative Results} Making \textsf{IE-System} work required a large
effort: to create the right training dataset, to configure the pipeline
correctly (\eg providing effective extraction rules), and to do so for each
relationship of interest. In contrast, \textsf{FabricQA-Extractor} only requires
one question template.



==> sections/old_rq6.tex <==
\subsection{RQ6: Sensitivity to Training Dataset Size}

We have demonstrated how, once trained on one dataset,
\textsf{FabricQA-Extractor} generalizes well to other domains. Here we explore
how hard it is to train it in the first place by studying its sensitivity to the
training dataset size.

We vary the training dataset size using two different strategies. In the first,
we create a training dataset by randomly sampling a given percentage of tuples
from each relationship. In the second, we fix the number of tuples per relation,
but vary the number of relations from where we sample. We also report results
when the model is not trained, as a reference baseline. We use the same test
data as in Section~\ref{section:rq5}.

%\item{Changing rows}. We keep all 84 relationships in the train data, but sample
%in each relationship 1\%, 5\%, 10\%, 15\%, 20\%, 25\% tuples (rows), where 1\%
%is 2208 rows and 25\% is 55307 rows. We make sure larger portion always includes
%smaller one.
%
%\item{Changing relationships}. We sample 98 (the maximum of one particular
%relationship in the train data) tuples first for each relationship to fix the
%rows. Then we sample relationships with step 10, and also make sure larger
%portion always includes smaller one. This results in 980 rows for 10
%relationships and 8232 rows for all 84 relationships.     
%
%\end{myitemize}
%
%We construct a special baseline, no data at all. To this end, we save the model
%immediately after initializing it. 

 
\mypar{Results} Table \ref{tab:row_efficiency} shows the result of the first
strategy. Without any data, \textsf{FabricQA-Extractor} achieves only 3.11/6.94 (EM/F1).
Using only 1\% of data (which corresponds to 2208 rows) results in 55.27/68.46
the biggest jump in performance. From then on, the table demonstrates the
diminishing returns of training data, with a maximum performance of 
56.24/69.3 when using 25\% rows per relationship. Table
\ref{tab:relation_efficiency} shows the results for the second strategy, where
we sample from increasingly more relationships. The trend is similar to the
previous, although with less diversity in the relationships, the results are
worse.

In summary, this results demonstrate that a small number of training samples is
sufficient to obtain good performance, and that, when possible, that training
dataset should be diverse in terms of the kinds of relationships it represents.

\notefb{R1-D9 - It's hard to compare the sample efficiency with changing rows versus relationsips in Tables 5 and 6 because the number of rows is not consistent. Is there a better way to visualize this?}

\noteqi{
We should emphasize changing rows and changing relationships are two perspectives and not comparable. 
}

%It shows the same trend as
%in changing rows. 10 relationships already achieves comparable result
%54.89/68.28 to that, 55.77/69.15 of all 84 relationships.

\begin{table}[ht]
\begin{tabular}{|c|c|c|c|c|c|}
\hline
\multicolumn{2}{|c|}{\textbf{Rows(Questions)}} & \multicolumn{2}{c|}{\textbf{FabricQA}} & \multicolumn{2}{c|}{\textbf{FabricQA-Extractor}} \\ \hline
\textbf{Percent}        & \textbf{Count}       & \textbf{EM}        & \textbf{F1}       & \textbf{EM}             & \textbf{F1}            \\ \hline
0                       & 0                    & 4.29               & 8.02              & 3.11                    & 6.94                   \\ \hline
0.1                     & 235                  & 53.81              & 66.76             & 54.92                   & 68.23                  \\ \hline
0.5                     & 1,121                & 54.44              & 67.54             & 55.32                   & 68.64                  \\ \hline
%1                       & 2,208                & 54.18              & 67.14             & 55.27                   & 68.46                  \\ \hline
5                       & 11,059               & 54.50              & 67.33             & 55.57                   & 68.73                  \\ \hline
%10                      & 22,121               & 54.7               & 67.68             & 56.15                   & 69.26                  \\ \hline
15                      & 33,183               & 55.13              & 67.93             & 56.04                   & 69.3                   \\ \hline
%20                      & 44,245               & 54.74              & 67.65             & 55.96                   & 69.03                  \\ \hline
25                      & 55,307               & 54.94              & 67.8              & 56.24                   & 69.3                   \\ \hline
\end{tabular}
\caption{Sample efficiency with changing rows}
\label{tab:row_efficiency}
\end{table}


\begin{table}[ht]
\begin{tabular}{|c|c|c|c|c|c|}
\hline
\multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Relation-\\ ships\end{tabular}}} & \multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Rows\\ (Questions)\end{tabular}}} & \multicolumn{2}{c|}{\textbf{FabricQA}} & \multicolumn{2}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}FabricQA-\\ Extractor\end{tabular}}} \\ \cline{3-6} 
                                                                                    &                                                                                      & \textbf{EM}        & \textbf{F1}       & \textbf{EM}                                  & \textbf{F1}                                  \\ \hline
0                                                                                   & 0                                                                                    & 4.29               & 8.02              & 3.11                                         & 6.94                                         \\ \hline
1                                                                                   & 98                                                                                   & 41.02              & 52.6              & 44.64                                        & 56.68                                        \\ \hline
5                                                                                   & 490                                                                                  & 51.18              & 64.23             & 52.52                                        & 65.58                                        \\ \hline
10                                                                                  & 980                                                                                  & 53.58              & 66.85             & 54.89                                        & 68.28                                        \\ \hline
20                                                                                  & 1,960                                                                                & 53.57              & 66.5              & 55.16                                        & 68.43                                        \\ \hline
%30                                                                                  & 2,940                                                                                & 54.18              & 67.04             & 55.57                                        & 68.77                                        \\ \hline
40                                                                                  & 3,920                                                                                & 54.12              & 66.94             & 55.55                                        & 68.88                                        \\ \hline
%50                                                                                  & 4,900                                                                                & 54.22              & 67.12             & 55.44                                        & 68.71                                        \\ \hline
%60                                                                                  & 5,880                                                                                & 54.5               & 67.37             & 55.59                                        & 68.93                                        \\ \hline
%70                                                                                  & 6,860                                                                                & 54.72              & 67.72             & 55.54                                        & 68.82                                        \\ \hline
84                                                                                  & 8,232                                                                                & 54.6               & 67.61             & 55.77                                        & 69.15                                        \\ \hline
\end{tabular}
\caption{Sample efficiency with changing relationships}
\label{tab:relation_efficiency}
\end{table}



==> sections/old_system_overview.tex <==
\section{\textsf{FabricQA-Extractor} Architecture}
\label{sec:overview}

\notera{explain how the details matter: i) they are not common in the
literature; ii) they are needed to make these systems work well, detials go
beyond the parameteres of the ml models}

In this section, we present the system architecture
in Section~\ref{subsec:architecture} and the user interaction model in
Section~\ref{subsec:ix}. 

\notera{system input: offline and online, say we've built a UI}

\notera{system pipeline -- this is fabricqa}

\notera{system output -- relation verifier, provenance, etc, say we've built a
UI}

\subsection{Input Interfaces and Setup}

\subsection{System Architecture}
\label{subsec:architecture}

The \textsf{FabricQA-Extractor} system architecture is shown in \F\ref{fig:architecture}.
This architecture is the result of several iterations. It consists of two
components:

\begin{figure}
  \centering
  \includegraphics[width=\columnwidth]{img/system_overview}
  \caption{\textsf{FabricQA-Extractor}'s architecture overview}
  \label{fig:architecture}
\end{figure}

\mypar{FabricQA} implements the \textsf{answer-this} primitive.
\textsf{FabricQA} takes as input a natural language question and a collection of
documents. It then finds a set of suitable passages, and for each passage, a
span of text that answers the question.  \textsf{FabricQA} may return the top-$K$ answers
and let clients select the right one. We explain \textsf{FabricQA} in detail in
Section~\ref{sec:fabricqa}, but here we highlight the cascade-based architecture
of its internal components. The more downstream a component, the more
sophisticated and the more computationaly expensive it is.  Hence, as data flows
downstream, it is increasingly filtered out by each component. As a result, the
system achieves high processing throughput. 

\mypar{Relation-Coherence} The Relation-Coherence is a trained model. It is 
explained in detail in Section~\ref{sec:relver}. Given a
table with missing cells as in \F\ref{fig:diagram} and a collection
of top-K answers for each missing cell, this model predicts the most likely
answer. To achieve that it uses information from the question, the object, the
relationship, the passage, and, crucially, relational information such as other
rows and other columns. 

\smallskip

\textsf{FabricQA-Extractor} has an offline stage and an online stage.

\mypar{Offline stage} In the \textsf{FabricQA} offline stage, documents are split into
passages according to a splitting criteria, and then indexed into an information
retrieval system. During the Relation-Coherence offline stage, the model is
trained using a training dataset of questions, passages, and answers. 

\mypar{Online stage} During the online stage, \textsf{FabricQA} serves requests, which
take the form of a natural question, used to retrieve the top-K answers from the
document corpora. Relation-Coherence first obtains the top-K answers for each
missing cell of the input table. Then it computes the most likely result per
cell and returns the results to the user.

\notera{move this to the intro of this section instead, before explaining the
system}
\mypar{Design Goals} There are 4 metrics that drive the design of this system.
\emph{Accuracy:} we design the system to achieve good quality results,
measured in number of correct answers. \emph{Scalability:} The system must work
even on corpora of millions of documents. \emph{Throughput:} We want to answer
questions with subsecond latencies to make the system use practical.
\emph{Transparency:} The system consists of a complex pipeline of components. We
strive to attach context (document, passage, answer, scores) to each provided
answer to facilitate the system's use.

\subsection{User Interaction Model}
\label{subsec:ix}

\mypar{Input} To use \textsf{FabricQA-Extractor}, users provide a partially filled table
and a question template per partially filled table attribute, as explained in
Section~\ref{subsec:setting} and illustrated in \F\ref{fig:diagram}. Users can
provide handcrafted questions for each row if they wish. We use the template
approach in the evaluation section, since it is the one that demands lower
effort from users.

\mypar{Output} After submitting table and question template,
\textsf{FabricQA-Extractor}
returns the filled in table. Users can inspect each newly filled cell. On
inspection, they have access to the lineage of that answer: the set of candidate
answers from where it was chosen, the passage where it was extracted from, and
the document where that passage belongs. Exposing this provenance information to
users helps make the system's results more interpretable. Each filled in value
is associated with a system-specific confidence score\footnote{This does not
correspond to confidence in the statistical sense, it is rather an informative
value that help users understand the amount of evidence the system had to
produce an answer.}, which helps users determine quickly what answers may be
worth inspecting in greater detail.

\mypar{What if subjects are unknown?} Users can use \textsf{FabricQA} to populate the
subjects before filing other columns with \textsf{FabricQA-Extractor}. For example, they
can ask \emph{"what are names of countries?"}, to quickly collect a list of countries over
which they can further ask other questions by adding the appropriate columns to
the table and the question templates.



